Fast Primal-Dual Gradient Method for Strongly Convex Minimization Problems with Linear Constraints

In this paper we consider a class of optimization problems with a strongly convex objective function and the feasible set given by an intersection of a simple convex set with a set given by a number of linear equality and inequality constraints. A number of optimization problems in applications can be stated in this form, examples being the entropy-linear programming, the ridge regression, the elastic net, the regularized optimal transport, etc. We extend the Fast Gradient Method applied to the dual problem in order to make it primal-dual so that it allows not only to solve the dual problem, but also to construct nearly optimal and nearly feasible solution of the primal problem. We also prove a theorem about the convergence rate for the proposed algorithm in terms of the objective function and the linear constraints infeasibility.

==> DOOR 2016 (2016-05-10) - final - for arxiv/pics2016-04-28/2err_2_0.tex <==
\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|}
    \hline
&\multicolumn{2}{|c}{FGM} &\multicolumn{2}{|c}{BAL} &\multicolumn{2}{|c}{CGM} &\multicolumn{2}{|c}{REG} \\
\hline
 $\varepsilon^{rel}$ &  Iterations &  Time &  Iterations &  Time &  Iterations &  Time &  Iterations &  Time \\
 \hline
 0.001 &15963& 23.05 &5326& 2.83 &12444& 68.28 &1443434& 164.00 \\
 0.002 &13268& 23.18 &3237& 2.03 &8191& 52.22 &998871& 124.43 \\
 0.003 &8544& 14.47 &7512& 4.35 &11194& 65.15 &1307046& 161.14 \\
 0.004 &8533& 14.22 &4681& 2.59 &7315& 37.35 &946386& 112.20 \\
 0.005 &6497& 10.51 &2806& 1.52 &11488& 51.56 &706271& 83.76 \\
 0.006 &5844& 9.53 &17641& 9.56 &13052& 55.16 &642863& 78.63 \\
 0.007 &6333& 9.65 &8391& 4.53 &34219& 145.13 &495646& 58.66 \\
 0.008 &5411& 8.30 &4554& 2.47 &11649& 48.79 &899095& 107.79 \\
 0.009 &5524& 8.36 &2370& 1.28 &45330& 167.23 &552173& 63.36 \\
 0.01 &4547& 5.69 &1948& 0.93 &29222& 94.30 &439564& 44.25 \\
\hline
\end{tabular}

==> DOOR 2016 (2016-05-10) - final - for arxiv/pics2016-04-28/dim_iter.tex <==
\begin{tabular}{|c|c||c|c|c|c|c|c|c|c|}
	\hline
 &Dimension & 16 & 81 & 256 & 625 & 1296 & 2401 & 4096 & 6561 \\
FGM & Iterations & 345 & 498 & 645 & 967 & 1260 & 1492 & 1999 & 2597 \\
FGM & Time & 0.28 & 0.41 & 0.68 & 1.39 & 3.70 & 14.79 & 36.66 & 109.68 \\
BAL & Iterations & 67 & 238 & 345 & 492 & 658 & 1015 & 1308 & 1250 \\
BAL & Time & 0.02 & 0.06 & 0.12 & 0.26 & 0.66 & 1.91 & 3.95 & 5.83 \\
CGM & Iterations & 173 & 356 & 245 & 300 & 373 & 264 & 337 & 334 \\
CGM & Time & 0.29 & 0.51 & 0.49 & 0.86 & 2.96 & 9.04 & 23.43 & 52.85 \\
REG & Iterations & 5421 & 6779 & 19330 & 32702 & 68330 & 109211 & 137243 & 132101 \\
REG & Time & 0.27 & 0.40 & 1.80 & 3.46 & 12.86 & 51.28 & 168.69 & 288.71 \\
	\hline
\end{tabular}


==> pics2016-04-28/2err_2_0.tex <==
\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|}
    \hline
&\multicolumn{2}{|c}{FGM} &\multicolumn{2}{|c}{BAL} &\multicolumn{2}{|c}{CGM} &\multicolumn{2}{|c}{REG} \\
\hline
 $\varepsilon^{rel}$ &  Iterations &  Time &  Iterations &  Time &  Iterations &  Time &  Iterations &  Time \\
 \hline
 0.001 &15963& 23.05 &5326& 2.83 &12444& 68.28 &1443434& 164.00 \\
 0.002 &13268& 23.18 &3237& 2.03 &8191& 52.22 &998871& 124.43 \\
 0.003 &8544& 14.47 &7512& 4.35 &11194& 65.15 &1307046& 161.14 \\
 0.004 &8533& 14.22 &4681& 2.59 &7315& 37.35 &946386& 112.20 \\
 0.005 &6497& 10.51 &2806& 1.52 &11488& 51.56 &706271& 83.76 \\
 0.006 &5844& 9.53 &17641& 9.56 &13052& 55.16 &642863& 78.63 \\
 0.007 &6333& 9.65 &8391& 4.53 &34219& 145.13 &495646& 58.66 \\
 0.008 &5411& 8.30 &4554& 2.47 &11649& 48.79 &899095& 107.79 \\
 0.009 &5524& 8.36 &2370& 1.28 &45330& 167.23 &552173& 63.36 \\
 0.01 &4547& 5.69 &1948& 0.93 &29222& 94.30 &439564& 44.25 \\
\hline
\end{tabular}

==> pics2016-04-28/dim_iter.tex <==
\begin{tabular}{|c|c||c|c|c|c|c|c|c|c|}
	\hline
 &Dimension & 16 & 81 & 256 & 625 & 1296 & 2401 & 4096 & 6561 \\
FGM & Iterations & 345 & 498 & 645 & 967 & 1260 & 1492 & 1999 & 2597 \\
FGM & Time & 0.28 & 0.41 & 0.68 & 1.39 & 3.70 & 14.79 & 36.66 & 109.68 \\
BAL & Iterations & 67 & 238 & 345 & 492 & 658 & 1015 & 1308 & 1250 \\
BAL & Time & 0.02 & 0.06 & 0.12 & 0.26 & 0.66 & 1.91 & 3.95 & 5.83 \\
CGM & Iterations & 173 & 356 & 245 & 300 & 373 & 264 & 337 & 334 \\
CGM & Time & 0.29 & 0.51 & 0.49 & 0.86 & 2.96 & 9.04 & 23.43 & 52.85 \\
REG & Iterations & 5421 & 6779 & 19330 & 32702 & 68330 & 109211 & 137243 & 132101 \\
REG & Time & 0.27 & 0.40 & 1.80 & 3.46 & 12.86 & 51.28 & 168.69 & 288.71 \\
	\hline
\end{tabular}

